Weak in the NEES?: Auto-tuning Kalman Filters with Bayesian Optimization

Kalman filters are routinely used for many data fusion applications including navigation, tracking, and simultaneous localization and mapping problems. However, significant time and effort is frequently required to tune various Kalman filter model parameters, e.g. process noise covariance, pre-whitening filter models for non-white noise, etc. Conventional optimization techniques for tuning can get stuck in poor local minima and can be expensive to implement with real sensor data. To address these issues, a new "black box" Bayesian optimization strategy is developed for automatically tuning Kalman filters. In this approach, performance is characterized by one of two stochastic objective functions: normalized estimation error squared (NEES) when ground truth state models are available, or the normalized innovation error squared (NIS) when only sensor data is available. By intelligently sampling the parameter space to both learn and exploit a nonparametric Gaussian process surrogate function for the NEES/NIS costs, Bayesian optimization can efficiently identify multiple local minima and provide uncertainty quantification on its results.

==> KalmanFilter_background.tex <==

More formally, let 
\begin{align}
\ex{k}  &= \xCond{k}{k} - \x{k}, \\
\ez{k}  &= \zCond{k}{k-1} - \z{k},
\end{align}
be the state estimation error and measurement residual (innovation) at time $k$, respectively. 

However, the filter statistics : if the system models are linear, precise knowledge of the process and observation models (including their noise characteristics) must be known. If the systems are nonlinear, exact solutions rarely exist and most approximations introduce a bias at some level. 



When in the presence of a mismatched filter, 

...relevant prior work: hand-tuning, stuff on id'ing KF/SS model and tuning params: max likelihood tuning, etc. for id'ing process/measurement noises from data...caveats: need lots of data, not easy for nonlinear systems, etc.
%%




